SecuRe -- An Approach to Recommending Security Design Patterns

Security is an important quality of software systems, but there is a huge lack of security experts. To overcome this gap, we aim to make security design knowledge reusable for architects by proposing the SecuRe recommendation approach to secure software design. It lifts design patterns and knowledge engineering concepts to security-related design recommendations for software architectures. This paper presents the central concepts of this approach, the overall recommendation process, and the first results from an initial case study.

==> tables/RCs_expected_under_each_RC_borders.tex <==
\begin{table}[t]
\caption{Realization contexts and expected recommendations}
\label{tab:evaluation_config}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{lllllll}
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Realization}\\ \textbf{Contexts}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{requir.}\\ \code{securty}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{requir.}\\ \code{usablty}\end{tabular}} & \multicolumn{1}{l|}{\code{budget}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{no.}\\ \code{users}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{intern/}\\ \code{extern}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\code{shared}\\ \code{device}\end{tabular} \\ \hline \hline

\multicolumn{1}{l|}{\textbf{RC1}} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{internal}& no \\ \cline{2-7} 
\multicolumn{7}{l}{\textit{expected best SPs:} \code{passkey}, \code{biom-device}, and \code{biom-profile}}\\ \hline

\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal} & no\\ 
\cline{2-7} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{passkey}, \code{biom-device}, and \code{biom-profile}} \\ \hline
\multicolumn{1}{l|}{\textbf{RC3}}                         & \multicolumn{1}{l|}{high}                                              & \multicolumn{1}{l|}{low}                                                 & \multicolumn{1}{l|}{high}                         & \multicolumn{1}{l|}{low}                                                & \multicolumn{1}{l|}{internal}                                                & no                                                  \\ \cline{2-7} 
\multicolumn{7}{l}{\textit{expected best SPs:} \code{passkey}, \code{biom-device}, and \code{biom-profile}}                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal}                        & no                                                  \\ \cline{2-7} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{password}}                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{\textbf{RC5}}                         & \multicolumn{1}{l|}{low}                                               & \multicolumn{1}{l|}{high}                                                & \multicolumn{1}{l|}{low}                          & \multicolumn{1}{l|}{high}                                               & \multicolumn{1}{l|}{internal}                                                & no                                                  \\ \cline{2-7} 
\multicolumn{7}{l}{\textit{expected best SPs:} \code{password}}                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                      & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal}                        & yes                                                 \\ \cline{2-7} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{biom-profile} or \code{key-stretch}}                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\multicolumn{1}{l|}{\textbf{RC7}}                         & \multicolumn{1}{l|}{low}                                               & \multicolumn{1}{l|}{low}                                                 & \multicolumn{1}{l|}{high}                         & \multicolumn{1}{l|}{low}                                                & \multicolumn{1}{l|}{external}                                                & no                                                  \\ \cline{2-7} 
\multicolumn{7}{l}{\textit{expected best SPs:} \code{passkey}, \code{biom-device}, and \code{biom-profile}}                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}external}                        & yes                                                 \\ \cline{2-7} 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{password} or \code{biom-profile}}                                                                                                                                                                                                                                                                                                                                                                                        
\end{tabular}
}
\end{table}

==> tables/RCs_expected_under_each_RC_no_borders.tex <==
\begin{table}[t]
\caption{Realization contexts and expected recommendations}
\label{tab:evaluation_config}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{lllllll}
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Realization}\\ \textbf{Contexts}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{requir.}\\ \code{securty}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{requir.}\\ \code{usablty}\end{tabular}} & \multicolumn{1}{l|}{\code{budget}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{no.}\\ \code{users}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{intern/}\\ \code{extern}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\code{shared}\\ \code{device}\end{tabular} \\ \hline \hline

\multicolumn{1}{l|}{\textbf{RC1}} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{internal}& no \\
\multicolumn{7}{l}{\textit{expected best SPs:} \code{passkey}, \code{biom-device}, \code{biom-profile}}\\ \hline

\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC2}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal} & no\\ 
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{passkey}, \code{biom-device}, \code{biom-profile}} \\ \hline
\multicolumn{1}{l|}{\textbf{RC3}}                         & \multicolumn{1}{l|}{high}                                              & \multicolumn{1}{l|}{low}                                                 & \multicolumn{1}{l|}{high}                         & \multicolumn{1}{l|}{low}                                                & \multicolumn{1}{l|}{internal}                                                & no                                                  \\
\multicolumn{7}{l}{\textit{expected best SPs:} \code{passkey}, \code{biom-device}, \code{biom-profile}}                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC4}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal}                        & no                                                  \\  
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{password}}                                                                                                                                                                                                                                                                                                                                                                                                         \\ \hline
\multicolumn{1}{l|}{\textbf{RC5}}                         & \multicolumn{1}{l|}{low}                                               & \multicolumn{1}{l|}{high}                                                & \multicolumn{1}{l|}{low}                          & \multicolumn{1}{l|}{high}                                               & \multicolumn{1}{l|}{internal}                                                & no                                                  \\  
\multicolumn{7}{l}{\textit{expected best SPs:} \code{password}}                                                                                                                                                                                                                                                                                                                                                                                                                                 \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC6}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                      & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal}                        & yes                                                 \\  
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{biom-profile} or \code{key-stretch}}                                                                                                                                                                                                                                                                                                                                                                                      \\ \hline
\multicolumn{1}{l|}{\textbf{RC7}}                         & \multicolumn{1}{l|}{low}                                               & \multicolumn{1}{l|}{low}                                                 & \multicolumn{1}{l|}{high}                         & \multicolumn{1}{l|}{low}                                                & \multicolumn{1}{l|}{external}                                                & no                                                  \\  
\multicolumn{7}{l}{\textit{expected best SPs:} \code{passkey}, \code{biom-device}, \code{biom-profile}}                                                                                                                                                                                                                                                                                                                                                                                                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
\multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}\textbf{RC8}} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                       & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                         & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}  & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low}                        & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}external}                        & yes                                                 \\  
\rowcolor[HTML]{EFEFEF} 
\multicolumn{7}{l}{\cellcolor[HTML]{EFEFEF}\textit{expected best SPs:} \code{password} or \code{biom-profile}}                                                                                                                                                                                                                                                                                                                                                                                        
\end{tabular}
}
\end{table}

==> tables/backup-hl.tex <==
\begin{table}[t]
\caption{Realization contexts and expected recommendations}
\label{tab:evaluation_config}
\centering
    \resizebox{\linewidth}{!}{
\begin{tabular}{l|llllll}
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\textbf{RCs}\\ \textbf{Expectations}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{requir.}\\ \code{sec-lev}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{requir.}\\ \code{use-lev}\end{tabular}} & \multicolumn{1}{l|}{\code{budget}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{no.}\\ \code{users}\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}\code{intern/}\\ \code{extern}\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\code{shared}\\ \code{device}\end{tabular} \\ \hline \hline
 & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{internal} & no \\ \cline{2-7}
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}RC1\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\code{passkey}, \code{biom-device}, \code{biom-profile}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal} & no \\ \cline{2-7}
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}RC2\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\code{passkey}, \code{biom-device}, \code{biom-profile}} \\ \hline
 & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{internal} & no \\ \cline{2-7}
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}RC3\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\code{passkey}, \code{biom-device}, \code{biom-profile}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal} & no \\ \cline{2-7}
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}RC4\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\code{password}} \\ \hline
 & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{internal} & no \\ \cline{2-7}
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}RC5\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\code{password}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}high} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}internal} & yes \\ \cline{2-7}
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}RC6\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\code{biom-profile}} \\ \hline
 & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{high} & \multicolumn{1}{l|}{low} & \multicolumn{1}{l|}{external} & no \\ \cline{2-7}
\multirow{-2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}RC7\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\code{passkey}, \code{biom-device}, \code{biom-profile}} \\ \hline
\rowcolor[HTML]{EFEFEF} 
\cellcolor[HTML]{EFEFEF} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}low} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}external} & yes \\ \cline{2-7}
\rowcolor[HTML]{EFEFEF} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}\textbf{\begin{tabular}[c]{@{}l@{}}RC8\\ exp. best SPs:\end{tabular}}} & \multicolumn{6}{l}{\cellcolor[HTML]{EFEFEF}\code{password} or \code{biom-profile}}
\end{tabular}
}
\end{table}
